REVAMP$^2$T: Real-time Edge Video Analytics for Multi-camera Privacy-aware Pedestrian Tracking

This article presents REVAMP$^2$T, Real-time Edge Video Analytics for Multi-camera Privacy-aware Pedestrian Tracking, as an integrated end-to-end IoT system for privacy-built-in decentralized situational awareness. REVAMP$^2$T presents novel algorithmic and system constructs to push deep learning and video analytics next to IoT devices (i.e. video cameras). On the algorithm side, REVAMP$^2$T proposes a unified integrated computer vision pipeline for detection, re-identification, and tracking across multiple cameras without the need for storing the streaming data. At the same time, it avoids facial recognition, and tracks and re-identifies pedestrians based on their key features at runtime. On the IoT system side, REVAMP$^2$T provides infrastructure to maximize hardware utilization on the edge, orchestrates global communications, and provides system-wide re-identification, without the use of personally identifiable information, for a distributed IoT network. For the results and evaluation, this article also proposes a new metric, Accuracy$\cdot$Efficiency (\AE), for holistic evaluation of IoT systems for real-time video analytics based on accuracy, performance, and power efficiency. REVAMP$^2$T outperforms current state-of-the-art by as much as thirteen-fold \AE~improvement.

==> tex/biography.tex <==
\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./figs/bio/Neff2}}]{Christopher Neff}
(S’18) 
received a B.S. in Computer Engineering
from the University of Carolina at Charlotte, Spring of 2019. He is currently pursuing a Ph.D. in Electrical Engineering under the mentorship of Dr. Hamed Tabkhi. His area of research is focused on enabling real-time artificial intelligence on low-power edge devices. This includes architecture and algorithmic co-design, system-level optimization, and end-to-end development with regards to power, scalability, and latency requirements.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./figs/bio/Matias.jpg}}]{Mat\'{i}as Mendieta}
(S’17)
is a M.S. student in the TeCSAR laboratory at the University of North Carolina at Charlotte (UNCC), advised by Dr. Hamed Tabkhi. He received his B.S. degree in Computer Engineering from UNCC in the spring of 2019. His research interests are in the areas of computer vision, deep learning, and robotics. These include perception algorithm development, performance optimization through hardware/software co-design, and enabling real-time, intelligent systems.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./figs/bio/shrey_img.jpg}}]{Shrey Mohan}
(S’18) is a Ph.D. student at the University of North Carolina at Charlotte (UNCC). He received his bachelor's in electronics and communications from the College of Technology, Pantnagar, India and his master's in computer engineering from UNCC. Currently, His research interests involve deep learning, computer vision, and edge computing, focusing on optimizing deep learning algorithms for embedded platforms. 
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./figs/bio/baharani}}]{Mohammadreza Baharani} (S’18) received the M.Sc. degree in computer engineering from University of Tehran, Iran, in 2012. He is currently a graduate research assistant and  Ph.D. student in the TeCSAR group, University of North Carolina at Charlotte, USA. His research goal is to solve real problems related to the intersection of computer architecture engineering and machine learning, in particular, hardware modeling and implementation of convolutional/recurrent neural networks.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./figs/bio/SamRogers.jpg}}]{Samuel Rogers}
(S'18) received a B.Sc. in Computer Engineerings from the University of North Carolina at Charlotte in the Spring of 2018. He is currently a graduate research assistant and Ph.D. student in Electrical Engineering at the University of North Carolina at Chalotte. His research is focused on computer architecture and systems modeling, as well as hardware-oriented code generation and optimization. In particular his focus is on mapping deep learning applications to the embedded domain.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./figs/bio/Hamed_Tabkhi.JPG}}]{Hamed Tabkhi}
(S’07–M’14)
is an Assistant Professor in the Department of Electrical and Computer Engineering, University of North Carolina at Charlotte, USA.
He was a post-doctoral research associate at Northeastern University. Hamed Tabkhi received his Ph.D. degree in 2014 from Northeastern University under the direction of Prof. Gunar Schirner. Overall, his research focuses on transformative computer systems and architecture for cyber-physical, real-time streaming and emerging machine learning applications.
\end{IEEEbiography}
